LHCb Open Data Ntupling Service: On-demand production and publishing of custom LHCb Open Data

The LHCb Ntupling Service enables on-demand production and publishing of LHCb Run 2 Open Data and aims at publishing them through the CERN Open Data Portal. It integrates the LHCb Ntuple Wizard to generate the configuration files that link custom user requests to the internal LHCb production system. User requests are managed through a streamlined workflow, from request creation to the final production of ROOT Ntuples, which can be downloaded directly from the Ntupling Service web interface, eliminating the need of running complex experiment-level software on the user side.

==> release.tex <==
\label{Release}
